Channel-Combination Algorithms for Robust Distant Voice Activity and Overlapped Speech Detection

Voice Activity Detection (VAD) and Overlapped Speech Detection (OSD) are key pre-processing tasks for speaker diarization. In the meeting context, it is often easier to capture speech with a distant device. This consideration however leads to severe performance degradation. We study a unified supervised learning framework to solve distant multi-microphone joint VAD and OSD (VAD+OSD). This paper investigates various multi-channel VAD+OSD front-ends that weight and combine incoming channels. We propose three algorithms based on the Self-Attention Channel Combinator (SACC), previously proposed in the literature. Experiments conducted on the AMI meeting corpus exhibit that channel combination approaches bring significant VAD+OSD improvements in the distant speech scenario. Specifically, we explore the use of learned complex combination weights and demonstrate the benefits of such an approach in terms of explainability. Channel combination-based VAD+OSD systems are evaluated on the final back-end task, i.e. speaker diarization, and show significant improvements. Finally, since multi-channel systems are trained given a fixed array configuration, they may fail in generalizing to other array set-ups, e.g. mismatched number of microphones. A channel-number invariant loss is proposed to learn a unique feature representation regardless of the number of available microphones. The evaluation conducted on mismatched array configurations highlights the robustness of this training strategy.

==> 99_backup.tex <==
\begin{table*}[h]
\centering
\caption{OSD performance on the Array1 of the AMI meeting corpus with the SACC system with a varying number of input channels.}
\begin{tabular}{@{}lcccccc@{}}
\toprule
AMI Array 1       & \multicolumn{2}{c}{F1-score (\%)}           & \multicolumn{2}{l}{Precision (\%)} & \multicolumn{2}{l}{Recall (\%)} \\ \midrule
$M=8$                & Dev  & Eval & Dev  & Eval & Dev & Eval \\ \cmidrule(lr){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} 
$STFT$                          & 72.4 & 68.8 & 72.5 & 72.8 & 72.3 & 65.2\\
$STFT$ w/ $\mathcal{L}_{inv}$    & \textbf{73.3} & \textbf{69.5} & \textbf{75.0} & \textbf{77.1} & \textbf{71.6} & \textbf{63.2}\\
$\mathcal{A}_{256}$             & 67.7 & 59.4 & 66.4 & 73.9 & 69.0 & 49.8\\
$\mathcal{A}_{256}$ \hfill w/ $\mathcal{L}_{inv}$     & 70.1 & 64.6 & 71.8 & \textbf{74.2} & 68.5 & 57.2\\ \midrule
$M=4$                & Dev  & Eval & Dev  & Eval & Dev & Eval \\ \cmidrule(lr){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} 
$STFT$                          & 45.0 & 41.4 & 41.2 & 36.5 & 49.6 & 47.7\\
$STFT$ w/ $\mathcal{L}_{inv}$    & \textbf{70.1} & \textbf{67.8} & \textbf{70.1} & \textbf{72.0} & \textbf{68.9} & 64.0\\
$\mathcal{A}_{256}$             & 43.8 & 42.8 & 30.9 & 29.8 & 75.8 & 75.9\\ 
$\mathcal{A}_{256}$ \hfill w/ $\mathcal{L}_{inv}$     & \textbf{70.0} & \textbf{65.1} & \textbf{71.4} & \textbf{74.0} & \textbf{68.7} & 58.0\\ \midrule
$M=2$                & Dev  & Eval & Dev  & Eval & Dev & Eval \\ \cmidrule(lr){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} 
$STFT$                        & 27.7 & 33.2 & 46.0 & 47.7.0 & 19.9 & 25.5\\ 
$STFT$ w/ $\mathcal{L}_{inv}$  & \textbf{70.6} & \textbf{67.6} & \textbf{71.1} & \textbf{69.1} & \textbf{70.1} & \textbf{66.0}\\ 
$\mathcal{A}_{256}$            & 0.18 & - & 0.12 & - & 100.0 & -\\ 
$\mathcal{A}_{256}$ \hfill w/ $\mathcal{L}_{inv}$     & \textbf{69.7} & \textbf{65.4} & \textbf{71.1} & \textbf{73.4} & \textbf{68.5} & 59.1\\
\bottomrule
\end{tabular}
\label{tab:array1-var_channels}
\end{table*}


\section{Old tables}

\begin{table}[b]
\centering
\caption{VAD performance of both BLSTM and TCN models with different front-ends.}
\begin{tabular}{@{}llcccccc@{}}
\toprule
    &   & \multicolumn{2}{c}{FA$_{\%\downarrow}$}           & \multicolumn{2}{l}{Miss$_{\%\downarrow}$} & \multicolumn{2}{l}{SER$_{\%\downarrow}$} \\ %\midrule
Front-end             & Model  & Dev  & Eval & Dev  & Eval & Dev & Eval \\ %\cmidrule(lr){2-3} \cmidrule(l){4-5} 
\midrule
Close-talk MFCC & BLSTM       & \textit{3.32} & \textit{3.12} & \textit{2.36} & \textit{2.61} & \textit{5.68} & \textit{5.70}\\ 
MFCC                & TCN      & \textit{3.14} & \textit{2.41} & \textit{2.69} & \textit{3.4} & \textit{5.83} & \textit{5.85}\\ \midrule
SDM             & BLSTM     & 4.07 & 2.08 & 2.80 & 6.29 & 6.88 & 8.38\\
MFCC            & TCN       & 4.76 & 2.95 & 1.82 & 3.99 & 6.57 & 6.95\\ \midrule
MVDR            & BLSTM     & 3.65 & 3.07 & 2.45 & 3.66 & 6.09 & 6.73\\ 
                & TCN       & 3.15 & 2.65 & 2.59 & 3.78 & \textbf{5.74} & \textbf{6.43}\\ \midrule                  
SACC            & BLSTM     & 3.52 & 3.07 & 2.43 & 3.55 & \textbf{5.95} & \textbf{6.62}\\ 
+$STFT$         & TCN       & 3.51 & 3.08 & 2.30 & 3.39 & \textbf{5.81} & \textbf{6.47}\\ \midrule
SACC            & BLSTM     & 3.98 & 3.26 & 2.98 & 4.49 & 6.96 & 7.75\\ 
+$\mathcal{A}_{256}$ & TCN  & 4.36 & 3.68 & 2.37 & 3.29 & 6.72 & 6.97\\ \midrule
IcSACC          & BLSTM     & 4.14 & 3.45 & 2.41 & 3.65 & 6.55 & 7.10\\ 
                & TCN       & 3.96 & 3.70 & 2.23 & 3.09 & 6.19 & 6.78\\ \midrule
EcSACC          & BLSTM     & 3.75 & 3.19 & 2.25 & 3.39 & \textbf{6.00} & \textbf{6.58}\\ 
                & TCN       & 3.78 & 3.23 & 2.09 & 3.16 & \textbf{5.87} & \textbf{6.39}\\ \bottomrule
\end{tabular}
\label{tab:vad_blstm_tcn}
\end{table}

\begin{comment}
\begin{table}[htbp]
\centering
\caption{VAD performance with both 2-class BLSTM and TCN architectures with each front-end. The scores in italics indicate the close-talk baseline.}
\begin{tabular}{@{}lccccccc@{}}
\toprule
  &                   & \multicolumn{2}{c}{F1-score (\%)}           & \multicolumn{2}{l}{Precision (\%)} & \multicolumn{2}{l}{Recall (\%)} \\ %\midrule
Front-end & Model  & Dev  & Eval & Dev  & Eval & Dev & Eval \\ %\cmidrule(lr){2-3} \cmidrule(l){4-5} 
\midrule
Close-talk & BLSTM  & \textit{96.7} & \textit{96.7} & \textit{96.2} & \textit{96.5} & \textit{97.3} & \textit{97.0}\\
MFCC       & TCN    & \textit{96.6} & \textit{96.6} & \textit{96.4} & \textit{97.2} & \textit{96.9} & \textit{96.1}\\ \midrule
SDM        & BLSTM  & 96.1 & 95.2 & 95.4 & 97.6 & 96.8 & 93.0\\
MFCC       & TCN    & 96.3 & 96.1 & 94.7 & 96.6 & 98.0 & 95.5\\ \midrule
MVDR       & BLSTM  & 96.5 & 96.2 & 95.9 & 96.5 & 97.2 & 95.9\\ 
            & TCN   & 96.7 & 96.3 & 96.4 & 96.9 & 97.0 & 95.5\\ \midrule
SACC       & BLSTM  & 96.6 & 96.2 & 96.0 & 96.5 & 97.2 & 96.0\\
+$STFT$    & TCN    & 96.4 & 96.3 & 95.2 & 96.5 & 97.7 & 96.2\\ \midrule
SACC       & BLSTM  & 96.0 & 95.6 & 95.5 & 96.3 & 96.0 & 95.0\\ 
+$\mathcal{A}_{256}$ & TCN & 96.0 & 96.1 & 95.1 & 95.9 & 96.9 & 96.3\\ \midrule
IcSACC    & BLSTM & 96.3 & 96.0 & 95.3 & 96.1 & 97.2 & 95.9\\ 
Mag-$\phi$ & TCN & 96.5 & 96.2 & 95.5 & 95.8 & 97.4 & 96.5\\ \midrule
EcSACC     & BLSTM & 96.6 & 96.3 & 95.7 & 96.4 & 97.4 & 96.2\\
 Mag-$\phi$  & TCN & 96.6 & 96.4 & 95.7 & 96.3 & 97.6 & 96.4\\
\bottomrule
\end{tabular}
\label{tab:vad_blstm_tcn}
\end{table}
\end{comment}

%The VAD performance between close-talk and distant speech is similar to the TCN model with only a 0.5\% absolute difference in F1-score.
%Although the performance between close-talk and distant speech are similar BLSTM VAD system shows similar performance with close-talk and distant speech material, the difference with the TCN is even smaller.
%The close talk VAD system shows comparative results with the BLSTM (96.6\%).
%Each distant system reaches at least~96.1\% F1-score on the evaluation set with the EcSACC system performing best with a 96.4\% F1-score. 
%Nevertheless, the performance gap between distant systems and the close-talk scenario does not exceed~0.5\%.
%This may be due to the better sequence modeling capacities of the TCN compared to the BLSTM~\cite{bai_empirical_2018}.

\begin{comment}
\begin{table}[htbp]
\centering
\caption{VAD performance using the TCN architecture with different preprocessing algorithms}
\begin{tabular}{@{}lcccccc@{}}
\toprule
       & \multicolumn{2}{c}{F1-score (\%)}           & \multicolumn{2}{l}{Precision (\%)} & \multicolumn{2}{l}{Recall (\%)} \\ %\midrule
AMI                       & Dev  & Eval & Dev  & Eval & Dev & Eval \\ %\cmidrule(lr){2-3} \cmidrule(l){4-5} 
\midrule
Close-talk MFCC        & \textit{96.6} & \textit{96.6} & \textit{96.4} & \textit{97.2} & \textit{96.9} & \textit{96.1}\\ \midrule
SDM MFCC               & 96.3 & 96.1 & 94.7 & 96.6 & 98.0 & 95.5\\
MVDR                   & 96.7 & 96.3 & 96.4 & 96.9 & 97.0 & 95.5\\ \midrule
SACC+$STFT$              & 96.4 & 96.3 & 95.2 & 96.5 & 97.7 & 96.2\\
SACC+$\mathcal{A}_{256}$          & 96.0 & 96.1 & 95.1 & 95.9 & 96.9 & 96.3\\ \midrule
IcSACC Mag-$\phi$                   & 96.5 & 96.2 & 95.5 & 95.8 & 97.4 & 96.5\\ 
EcSACC Mag-$\phi$                   & 96.6 & 96.4 & 95.7 & 96.3 & 97.6 & 96.4\\
\bottomrule
\end{tabular}
\label{tab:vad_tcn}
\end{table}
\end{comment}


\begin{table}[t]
\centering
\caption{OSD performance for both BLSTM and TCN architectures with each front-end algorithm.}
\begin{tabular}{@{}lccccccc@{}}
\toprule
  &                   & \multicolumn{2}{c}{F1-score$_{\%\uparrow}$}           & \multicolumn{2}{l}{Precision$_{\%\uparrow}$} & \multicolumn{2}{l}{Recall$_{\%\uparrow}$} \\ %\midrule
Front-end & Model  & Dev  & Eval & Dev  & Eval & Dev & Eval \\ %\cmidrule(lr){2-3} \cmidrule(l){4-5} 
\midrule
Close-talk & BLSTM     & \textit{70.3} & \textit{67.9} & \textit{68.9} & \textit{76.9} & \textit{71.8} & \textbf{60.9}\\
MFCC & TCN             & \textit{73.9} & \textit{70.2} & \textit{73.8} & \textit{81.4} & \textit{74.1} & \textit{61.8}\\ \midrule
SDM  & BLSTM         & 63.7 & 59.5 & 64.4 & 65.7 & 63.0 & 54.3\\
MFCC & TCN             & 68.8 & 65.5 & 69.5 & 72.8 & 68.1 & 59.5\\ \midrule
MVDR & BLSTM           & \textbf{68.8} & \textbf{65.3} & \textbf{68.0} & \textbf{71.9} & \textbf{69.6} & 59.9\\ 
     & TCN             & \textbf{72.1} & \textbf{69.5} & \textbf{74.3} & \textbf{73.1} & 70.0 & 66.2\\ \midrule
SACC & BLSTM           & \textbf{69.2} & \textbf{65.3} & \textbf{68.5} & 69.9 & \textbf{69.9} & \textbf{61.4}\\
+$STFT$ & TCN          & \textbf{72.4} & \textbf{68.8} & 72.5 & 72.9 & \textbf{72.3} & 65.2\\ \midrule
SACC & BLSTM        & 61.4 & 55.5 & 63.0 & 66.0 & 59.9 & 47.9\\
+$\mathcal{A}_{256}$ & TCN  & 67.8 & 62.9 & 66.4 & 67.4 & 69.0 & 58.9\\ \midrule
IcSACC & BLSTM                 & 63.9 & 59.0 & 61.9 & 70.2 & 66.0 & 50.9\\ 
            & TCN    & 69.1 & 64.8 & 69.4 & 74.5 & 68.6 & 57.4\\ \midrule
EcSACC       & BLSTM  & 66.8 & 63.7 & 68.8 & 72.5 & 64.9 & 56.8\\
             & TCN & \textbf{71.7} & 66.7 & 72.2 & 64.0 & 71.2 & \textbf{70.0}\\
\bottomrule
\end{tabular}
\label{tab:osd_blstm_tcn}
\end{table}


==> old_seg_results.tex <==
\section{Experimental results}
\label{5_sect_results_seg}

This section presents the VAD and OSD performance of both architectures with each front end.
Unless otherwise specified, all the mentioned scores are those obtained on the evaluation set (Eval).
The score comparisons are presented as absolute performance gain/degradation.

\subsection{Voice Activity Detection}

This section presents the VAD performance with each sequence modeling and front-end approach. %feature extractor.
The results obtained using BLSTM sequence modeling are presented in table~\ref{tab:vad_blstm_tcn}.
As expected, the close-talk system offers the best performance~(5.70\% SER) because of the higher signal quality with respect to the single-distant microphone (SDM) scenario.
In the latter case, evaluation SER is degraded by an absolute~+2.68\%(8.38\%).
The performance on distant speech can be improved by using multi-channel features with SACC~(6.62\%), EcSACC~(6.58\%), and IcSACC~(7.10\%) feature extractors.
The MVDR beamformer also offers similar performance as SACC-based models (6.73\%).
However, this algorithm requires estimating the noise covariance of the signal, which could be costly. 
%This algorithm however requires to estimate the noise covariance of the signal, which could be costly. 
Only the SACC algorithm based on analytic filters shows mitigated detection scores, offering similar results as the SDM case (7.75\%).


Table \ref{tab:vad_blstm_tcn} also presents the VAD performance of the TCN model. 
Although SDM performance is improved (6.95\% SER) compared to the BLSTM, it remains degraded with respect to the close-talk scenario (5.85\% SER).
This is mostly due to a high miss-detection rate in the SDM scenario (3.99\%).
MVDR (6.43\% SER) and SACC+$STFT$ (6.47\% SER) bring slight improvement with regard to the SDM scenario.
The EcSACC (6.39\% SER) reaches the best performance. 
However, IcSACC (6.88\%) and SACC+$\mathcal{A}_{256}$ (6.97\%) fail in improving distant VAD.

The use of channel combination algorithms can improve the VAD, mostly with the BLSTM architecture.
SACC+$STFT$ and EcSACC are good candidates for robust VAD.
The TCN-based VAD systems do not show a noticeable difference in performance.
Since a little in the VAD could change speaker diarization performance~ \cite{garcia_perera_speaker_2020}, these algorithms will be explored in speaker diarization systems front-ends in future work.
%The use of a specific algorithm for the VAD task in the distant speech scenario does not seem to be required according to the results obtained on the AMI dataset.
%The detection performance is close between the close-talk and the SDM cases.
%The use of multichannel algorithms like SACC may slightly increase the robustness of the system, with less performance degradation between the development and the test data.
%The use of these algorithms could probably be beneficial for speech materials that are more corrupted by noise and reverberation (e.g. CHiME-6 data~\cite{watanabe2020chime}).
%In summary, the results show that both BLSTM and TCN models are suitable for distant VAD.

\subsection{Overlapped Speech Detection}

This section presents the OSD performance of each front end using both BLSTM and TCN sequence modeling. 
OSD performance with both sequence modeling architectures is presented table~\ref{tab:osd_blstm_tcn}.
%OSD scores obtained with the BLSTM architecture are summarized in table \ref{tab:osd_blstm_tcn}. 
With the BLSTM architecture, the close-talk MFCC system reaches the best F1-score on both Dev (70.3\%) and Eval (67.9\%) sets because of the better signal quality. 
This system seems to show great generalization capacities with only -2.4\% degradation between Dev and Eval sets.
Furthermore, the single distant microphone (SDM) shows an~-8.4\% performance degradation with respect to the close-talk conditions with~59.5\% evaluation F1-score.
Moreover, the SDM model shows lower generalization capacities with a -4.2\% F1-score degradation between Dev and Eval sets. 
The performance degradation between distant speech and close talk is stronger than on the VAD task.
The MVDR beamformer reaches~65.3\% evaluation F1-score which represents~+5.8\% absolute gain compared to SDM.
This result was expected since beamforming enhances speech signals by spatially filtering out noise sources~\cite{benesty_microphone_2008}.
In the distant speech scenario, the use of a multi-channel front-end thus improves OSD.

The SACC+$STFT$ also noticeably improves OSD performance (65.3\%) under distant speech conditions with about~+5.3\% absolute F1-score improvement compared to the SDM scenario.
This model seems able to select the relevant information in the incoming channels.
The SACC+$STFT$ reaches a similar performance to the MVDR beamforming.
However, this algorithm does not require putting any assumption on the signal statistics since no covariance matrix estimation is needed.
The self-attention module learns from the raw STFT magnitude to efficiently combine the channels to improve OSD.

Replacing the STFT with a learnable filter bank does not bring significant improvement~(55.5\%) and even degrades distant OSD performance by -4\%.
The SACC+$\mathcal{A}_{256}$ fails in improving OSD in the distant speech scenario.
%The model does not seem able to learn filters to generate a discriminative feature sequence for the OSD task.
%The system does not seem able to learn filters with center frequencies higher than 1~kHz. (add figure)
%This approach will however be useful in order to learn an feature map invariant to the array geometry, as shown in Section \ref{6_sect_invariance}.\\
The two complex extensions of the SACC algorithm provide different outcomes. 
Results are presented considering the magnitude and phase formulation (see section~\ref{5_sect_csacc_detail}).
%In section~\ref{5_sect_csacc_detail}, we show that the magnitude and phase formulation offers better detection performance on the OSD task. 
%The OSD performance of both IcSACC and EcSACC is thus presented considering this formulation.
The IcSACC front-end shows similar results as the distant MFCC scenario~(59.0\%). 
Allowing the self-attention module to learn cross-relationships between magnitude and phase does not seem to improve distant OSD.
Nevertheless, the EcSACC system~(63.7\%) improves OSD with regard to the SDM scenario by~+4.2\%.
It seems beneficial to learn the magnitude and the phase separately for OSD, which simplifies the learning process.

For each system, the F1-score tends to decrease between the development and the evaluation sets.
This is mostly due to a mismatch between precision and recall.
Since the detection thresholds $\sigma_<$ and $\sigma_>$ are tuned on development data, they might not be optimal on the evaluation set.
This leads to a precision/recall mismatch.


The experiments conducted using the BLSTM model are reproduced with the TCN sequence modeling architecture (Table~\ref{tab:osd_blstm_tcn}).
Overall, the TCN architecture offers better OSD performance while the behavior of each front end remains the same.
%The conclusions about the OSD performance of each front-end within the TCN architecture are similar to the BLSTM ones.
For example, in the close-talk scenario, the TCN system reaches~70.2\% evaluation F1-score, an improvement of an absolute~+2.3\% with regard to the BLSTM model.
Under SDM conditions~(65.5\%), the TCN improves OSD by~+6\% compared to the BLSTM-based architecture~(59.5\%).
The SDM performance remains degraded compared to the close-talk scenario with a~-4.7\% F1-score degradation.

%To cope with this degradation, several multi-channel feature extractors are evaluated as OSD front end.
About multi-channel front-ends, the MVDR beamformer improves the detection performance with~69.5\% evaluation F1-score.
Again, SACC+$STFT$ improves the detection in the distant scenario~(68.8\%) compared to SDM.
%On the evaluation set, the SACC shows a slight drop in performance of~-0.7\% with respect to the MVDR beamforming. 
%This degradation is however compensated by the practical benefits of the SACC, which does not require any assumption on the signal statistics and avoids any covariance matrix estimation.
In spite of a -0.7\% drop in performance compared to MVDR, the SACC+$STFT$ remains suitable for distant OSD.

As with the BLSTM, SACC+$\mathcal{A}_{256}$ degrades the detection performance under distant speech conditions by an absolute~-2.6\% with regard to the SDM scenario.
This degradation is however mitigated compared to the BLSTM~(-4\%).
%This difference could be explained by the better sequence modeling abilities of the TCN compared to the BLSTM~\cite{bai_empirical_2018,Cornell2022}.

The two complex systems behave similarly to the BLSTM architecture.
On the one hand, the IcSACC algorithm~(64.8\%) offers similar results as the SDM system. 
Again, the system does not seem able to learn consistent combination weights from the concatenation of the magnitude and the phase.
On the other hand, the EcSACC algorithm~(66.7\%) shows closer OSD performance to SACC+$STFT$.
One can notice only~-0.7\% degradation on the development set compared to SACC+$STFT$. 
However, EcSACC seems less able to generalize shown by the gap between the development and the evaluation performance.
Although IcSACC and EcSACC do not drastically improve distant OSD performance, they still remain easier to interpret (see section~\ref{5_sect_csacc_detail}).
%The explainability of the model is thus improved as shown in~\cite{mariotte22_interspeech} and detailed in Section~\ref{5_sect_csacc_detail}.

As with the BLSTM architecture, there is a global performance mismatch between the development and the evaluation sets.
This is also a result of the detection thresholds not being optimized for the evaluation data.
The models show higher precision on the evaluation except for the EcSACC system which reaches 70.0\% recall and 64.0\% precision.

In summary, OSD performance degrades under distant speech conditions regardless of the type of sequence modeling architecture (BLSTM or TCN).
The use of a multi-channel front-end can improve detection under those conditions.
MVDR beamforming and SACC+$STFT$ show the best OSD performance on distant speech material.
However, the MVDR weight estimation requires a non-trivial additional step to estimate the noise covariance matrix of the input signal. 
The OSD performance is also improved with the EcSACC complex formulation.
However, neither SACC+$\mathcal{A}_{256}$ nor IcSACC improves the detection.

\begin{comment}
    


\begin{table}[htbp]
\centering
\caption{OSD performance using the TCN architecture with different front-ends}
\begin{tabular}{@{}lcccccc@{}}
\toprule
       & \multicolumn{2}{c}{F1-score (\%)}           & \multicolumn{2}{l}{Precision (\%)} & \multicolumn{2}{l}{Recall (\%)} \\ %\midrule
AMI                       & Dev  & Eval & Dev  & Eval & Dev & Eval \\ %\cmidrule(lr){2-3} \cmidrule(l){4-5} 
\midrule
Close-talk MFCC        & \textit{73.9} & \textit{70.2} & \textit{73.8} & \textit{81.4} & \textit{74.1} & \textit{61.8}\\ \midrule
SDM MFCC               & 68.8 & 65.5 & 69.5 & 72.8 & 68.1 & 59.5\\
MVDR                   & \textbf{72.1} & \textbf{69.5} & \textbf{74.3} & \textbf{73.1} & 70.0 & 66.2\\ \midrule
SACC+$STFT$              & \textbf{72.4} & \textbf{68.8} & 72.5 & 72.9 & \textbf{72.3} & 65.2\\
SACC+$\mathcal{A}_{256}$          & 67.8 & 62.9 & 66.4 & 67.4 & 69.0 & 58.9\\ \midrule
IcSACC Mag-$\phi$                   & 69.1 & 64.8 & 69.4 & 74.5 & 68.6 & 57.4\\ 
EcSACC Mag-$\phi$                   & \textbf{71.7} & 66.7 & 72.2 & 64.0 & 71.2 & \textbf{70.0}\\
\bottomrule
\end{tabular}
\label{tab:osd_tcn}
\end{table}




\subsection{VAD+OSD}

The previous sections have shown the VAD and OSD performance of 2-class models.
This section evaluates the joint training of both VAD and OSD with a 3-class model.
As with the 2-class system, each front-end is investigated. 
These models are evaluated on both VAD and OSD although both tasks are jointly trained.
The performance of the 3-class BLSTM and TCN models on the VAD and the OSD tasks is presented in tables~\ref{tab:3-classes_VAD} and~\ref{tab:3-classes_OSD} respectively.\\

\subsubsection{VAD}

The VAD performance of each 3-class model is presented in table~\ref{tab:3-classes_VAD}.
Joint VAD+OSD shows similar VAD scores as a single 2-class model. 
For example, in the close-talk scenario, the 3-class system shows~96.8\% and~96.9\% evaluation F1-score with BLSTM and TCN respectively.
This represents~0.2\% gap between the 2-~and 3-class models (see table~\ref{tab:vad_blstm_tcn}).

As with the 2-class approach, there is no significant difference in the VAD performance between the close-talk and the distant speech conditions.
This is observed for both BLSTM and TCN architectures.
Within the BLSTM system, MVDR~(96.4\%), SACC~(96.3\%), and EcSACC~(96.4\%) show the best VAD performance under distant conditions.
In contrast, SDM, analytical SACC, and IcSACC show a slight performance drop with~96.0\% evaluation F1-score.

TCN-based VAD+OSD shows a slight difference in the VAD performance compared to the BLSTM system.
Only the SACC+$STFT$ degrades VAD performance with 94.4\% evaluation F1-score.
Otherwise, SDM~(96.2\%), MVDR (96.5\%), IcSACC~(96.2\%) and SACC+$\mathcal{A}_{256}$~(96.2\%) show similar performance.
The EcSACC gets the best VAD performance on the evaluation set with 97.5\% F1-score and improves the BLSTM system by an absolute 1.1\%.\\


\begin{table}[htbp]
\centering
\caption{VAD performance of both 3-class BLSTM and TCN models with different front-end}
\begin{tabular}{@{}llcccccc@{}}
\toprule
    &   & \multicolumn{2}{c}{F1-score (\%)}           & \multicolumn{2}{l}{Precision (\%)} & \multicolumn{2}{l}{Recall (\%)} \\ %\midrule
Front-end             & Model  & Dev  & Eval & Dev  & Eval & Dev & Eval \\ %\cmidrule(lr){2-3} \cmidrule(l){4-5} 
\midrule
Close-talk & BLSTM       & \textit{96.3} & \textit{96.8} & \textit{94.1} & \textit{95.7} & \textit{98.5} & \textit{98.0}\\ 
MFCC                & TCN       & \textit{96.3} & \textit{96.9} & \textit{94.1} & \textit{97.0} & \textit{98.5} & \textit{96.8}\\ \midrule
SDM        & BLSTM       & 96.2 & 96.0 & 95.4 & 95.8 & 97.1 & 96.2\\
MFCC                & TCN       & 96.0 & 96.2 & 93.4 & 94.3 & 98.7 & 98.3\\ \midrule
MVDR            & BLSTM       & 96.7 & 96.4 & 95.5 & 95.9 & 97.9 & 97.0\\ 
                & TCN       & 96.6 & 96.5 & 94.9 & 95.5 & 98.4 & 97.5\\ \midrule                  
SACC            & BLSTM     & 96.6 & 96.3 & 95.4 & 95.6 & 97.8 & 97.0\\ 
+$STFT$         & TCN       & 96.6 & 94.4 & 95.8 & 96.4 & 97.4 & 96.5\\ \midrule
SACC            & BLSTM     & 95.9 & 96.0 & 93.5 & 94.3 & 98.3 & 97.7\\ 
+$\mathcal{A}_{256}$ & TCN  & 96.2 & 96.2 & 94.7 & 94.7 & 97.7 & 97.7\\ \midrule
IcSACC          & BLSTM     & 96.2 & 96.0 & 94.4 & 96.9 & 98.0 & 95.2\\ 
Mag-$\phi$      & TCN       & 96.0 & 96.2 & 93.9 & 95.2 & 98.2 & 97.3\\ \midrule
EcSACC          & BLSTM     & 96.7 & 96.4 & 95.8 & 96.5 & 97.5 & 96.2\\ 
Mag-$\phi$      & TCN       & 96.5 & 97.5 & 94.6 & 95.2 & 98.4 & 96.3\\ \bottomrule
\end{tabular}
\label{tab:3-classes_VAD}
\end{table}

\subsubsection{OSD}

The 3-class system is evaluated on the OSD task and results are presented in table~\ref{tab:3-classes_OSD}.
The BLSTM-based model has the same behavior as the 2-class approach (table~\ref{tab:osd_blstm}).
OSD performance in the SDM scenario (62.5\%) is degraded with respect to the close-talk configuration (69.2\%).
Again, both SACC+$\mathcal{A}_{256}$~(61.6\%) and IcSACC~(62.5\%) fail at improving distant OSD.
The IcSACC shows a high precision score on the evaluation set (68.3\%) in exchange for a decrease in the recall (57.6\%).
This shows the limited generalization capacities of this system.
However, MVDR~(66.9\%), EcSACC~(64.9\%) and SACC+$STFT$~(67.4\%) show interesting performance gain on distant speech.
The latter offers the best OSD performance for a BLSTM system.
In general, the joint VAD+OSD training improves the OSD performance of the BLSTM system.
For example, the F1-score is improved by an absolute +6.1\% with SACC+$\mathcal{A}_{256}$ scenario and by +2.1\% with SACC+$STFT$.

%The 3-classes model shows a slight improvement with the BLSTM architecture (table~\ref{tab:vad_osd_BLSTM}) on the OSD performance compared to the 2-classes formulation (table~\ref{tab:osd_blstm}). 
%With the BLSTM sequence modeling, OSD performance drops by~6.3\% between the close-talk and the SDM configurations, as observed with the 2-classes model.
%Moreover, the analytical SACC also fails at improving distant OSD with 61.6\% evaluation F1-score.
%The MVDR beamforming significantly improves OSD on multi-channel (66.9\%) data along with the original STFT-based SACC~(67.4\%).
%The latter shows the best distant OSD performance with the BLSTM architecture for both 2-~and 3-classes approaches, with a~+2.1\% gain compared to 2-classes BLSTM.
%About the complex systems, the 3-classes IcSACC~(62,5\%) does not show any improvement compared to the 3-classes SDM.
%However, the OSD performance is improved by~+3.5\% with respect to the 2-classes formulation (59.0\%).
%In contrast, the 3-classes EcSACC improves distant OSD~(64.9\%) and show better classification score than the 2-classes model (63.7\%).
%The use of a 3-classes approaches significantly improves the OSD performance with the BLSTM sequence modeling. 

The performance of the TCN-based 3-class model is presented in table~\ref{tab:3-classes_OSD}.
Except for the close-talk scenario (74.0\%), joint VAD+OSD does not improve the OSD performance with respect to the 2-class model.
The 3-class model shows similar performance.
The conclusions are thus the same, with the two best-performing systems being the MVDR ~(69.6\%) and the SACC+$STFT$~(67.9\%).
The EcSACC also shows an improvement of~+1.7\% with regard to the SDM scenario.
As with the 2-class model, the two other multi-channel approaches (SACC+$\mathcal{A}_{256}$ 62.7\%, IcSACC 63.9\%) do not show any significant improvement.

On most systems, there are noticeable mismatches between precision and recall on both development and evaluation sets.
For example, the close-talk TCN system shows 69.9\% precision and 78.8\% recall on the evaluation. 
Since there is no thresholding procedure with the 3-class system, the balance between precision and recall cannot be controlled.
The performance could probably be improved by adding detection thresholds.
This is however kept for future work.


\begin{table}[htbp]
\centering
\caption{OSD performance of both 3-class BLSTM and TCN models with each front-end}
\begin{tabular}{@{}llcccccc@{}}
\toprule
    &   & \multicolumn{2}{c}{F1-score (\%)}           & \multicolumn{2}{l}{Precision (\%)} & \multicolumn{2}{l}{Recall (\%)} \\ %\midrule
Front-end             & Model  & Dev  & Eval & Dev  & Eval & Dev & Eval \\ %\cmidrule(lr){2-3} \cmidrule(l){4-5} 
\midrule
Close-talk & BLSTM       & \textit{70.1} & \textit{69.2} & \textit{64.8} & \textit{72.8} & \textit{76.4} & \textit{66.0}\\ 
 MFCC                & TCN       & \textit{73.8} & \textit{74.0} & \textit{69.9} & \textit{76.9} & \textit{78.8} & \textit{71.3}\\ \midrule
SDM        & BLSTM       & 64.0 & 62.5 & 59.5 & 63.0 & 69.3 & 61.9\\
MFCC            & TCN       & 69.0 & 64.9 & 70.6 & 72.7 & 67.6 & 58.7\\ \midrule
MVDR            & BLSTM       & 68.5 & 66.9 & 64.0 & 70.7 & 73.7 & 63.5\\
                & TCN       & 72.3 & 69.6 & 72.5 & 77.0 & 72.3 & 63.6\\ \midrule
SACC     & BLSTM     & \textbf{70.2} & \textbf{67.4} & \textbf{69.2}& \textbf{71.9} & \textbf{71.1 }&\textbf{63.4}\\  
+$STFT$                  & TCN       & \textbf{71.8} & \textbf{67.9} & \textbf{74.5} & \textbf{76.0} & \textbf{69.3} & \textbf{61.4}\\ \midrule
SACC   & BLSTM       & 63.0 & 61.6 & 55.6 & 60.8 & 72.8 & 62.3\\ 
+$\mathcal{A}_{256}$ & TCN       & 66.6 & 62.7 & 62.7 & 63.9 & 70.9 & 61.6\\ \midrule 
IcSACC & BLSTM       & 65.1 & 62.5 & \textbf{63.4} & \textbf{68.3} & 66.9 & 57.6\\    
Mag-$\phi$         & TCN       & 69.3 & 63.9 & 70.5 & \textbf{75.3} & 68.1 & 55.4\\ \midrule
EcSACC   & BLSTM       & \textbf{66.3} & \textbf{64.9} & 61.4 & 64.7 & \textbf{71.9} &\textbf{65.0}\\
Mag-$\phi$                & TCN       & \textbf{71.3} & \textbf{66.6} & \textbf{71.5} & 73.8 & \textbf{71.1} & \textbf{60.6}\\ \bottomrule
\end{tabular}
\label{tab:3-classes_OSD}
\end{table}



In summary, the experiments conducted on the AMI corpus show that VAD and OSD can be jointly trained using a 3-class model.
This approach does not show any performance degradation on any of the tasks. 
The OSD performance is even improved when BLSTM sequence modeling is considered.
Joint VAD+OSD can thus be considered for each of the front-end algorithms. 
Considering these results, it could be preferable to implement a joint VAD+OSD system instead of two separated 2-class models for VAD and OSD in the meeting scenario.
The performance of the 3-class system could be improved by adding detection thresholds to control the precision/recall balance. 
This might be important to generate a robust speech segmentation in the context of speaker diarization.

\end{comment}
